Jets in Magnetically Arrested Hot Accretion Flows: Geometry, Power and Black Hole Spindown

We present the results of nine simulations of radiatively-inefficient magnetically arrested disks (MADs) across different values of the black hole spin parameter $a_*$: $-0.9$, $-0.7$, $-0.5$, $-0.3$, 0, 0.3, 0.5, 0.7, and 0.9. Each simulation was run up to $t \gtrsim 100,000\,GM/c^3$ to ensure disk inflow equilibrium out to large radii. We find that the saturated magnetic flux level, and consequently also jet power, of MAD disks depends strongly on the black hole spin, confirming previous results. Prograde disks saturate at a much higher relative magnetic flux and have more powerful jets than their retrograde counterparts. MADs with spinning black holes naturally launch jets with generalized parabolic profiles whose widths vary as a power of distance from the black hole. For distances up to $100\;GM/c^2$, the power-law index is $k \approx 0.27-0.42$. There is a strong correlation between the disk-jet geometry and the dimensionless magnetic flux, resulting in prograde systems displaying thinner equatorial accretion flows near the black hole and wider jets, compared to retrograde systems. Prograde and retrograde MADs also exhibit different trends in disk variability: accretion rate variability increases with increasing spin for $a_*>0$ and remains almost constant for $a_*\lesssim 0$, while magnetic flux variability shows the opposite trend. Jets in the MAD state remove more angular momentum from black holes than is accreted, effectively spinning down the black hole. If powerful jets from MAD systems in Nature are persistent, this loss of angular momentum will notably reduce the black hole spin over cosmic time.

==> extra.tex <==
\begin{figure}
	\includegraphics[width=8cm]{phi_r.pdf}
    \caption{Shows the variation of $\phi_{\rm BH}$ with radius $r$ for the nine simulations. Line types and colors are as in Fig. \ref{fig:rho_T}.}
    \label{fig:phi_r}
\end{figure}

\begin{figure*}
	\includegraphics[width=8cm]{Phi.pdf}
	\includegraphics[width=8cm]{rtMdot.pdf}
    \caption{Left: Total enclosed magnetic flux $\Phi$ vs $r$. Line types and colors are as in Fig. \ref{fig:profs1}. Right: $\sqrt{\dot{M}}$ vs $r$. }
    \label{fig:Phi_Mdot}
\end{figure*}

Ideas:
Figure \ref{fig:phi_r} shows how $\phi_{\rm BH}$ varies with $r$ for each of the nine simulations. The values at the horizon (left end of each curve) are what are shown in Figure \ref{fig:phi_MAD}. Not clear that this figure reveals anything interesting... \KC{Andrew, can you increase the x-axis to $1000r_g$? And is the y-axis $\Phi(r)/\sqrt{\dot{M}(r)}$? If we can show that the magnetic flux starts from the same level and becomes more and more smaller from large to small radii, then we can say that the transport of magnetic flux depends on BH spin.}\AC{I will try to make a plot that does this, it's a good idea. It might be trivial for Ramesh to extend the range in his script though}

\RN{Figure \ref{fig:Phi_Mdot} shows the magnetic flux $\Phi$ vs $r$ and the square root of $\dot{M}$ vs $r$ for the models. I went up to $r=100$, which is at the edge of inflow equilibrium (as the right panel shows). The $\Phi$ curves do converge at large radius. But there is also a curious behavior of $\dot{M}$. I think this story is muddy. Not clear it is useful. I would be tempted to eliminate Figures \ref{fig:phi_r} and \ref{fig:Phi_Mdot}.}

\KC{I'm not sure I understand the y-axis in Figure 11. $\phi_{\rm BH}=\phi/\sqrt{\dot{M}}\sim 10^{11.85}/10^{10.2}=44.67$ for the bold blue line at $\log r=0.5$. Is this the right way to interpret the plots? It looks like even though the prograde MADs show lower $\dot{M}$, their $\phi$ values are systematically higher at lower radii. Additionally $\dot{M}$ is very similar among the retrograde MADs, but $\phi$ still goes down. Doesn't that mean the inward flux transport is weaker (as in the slope is steeper) in retrograde MADs?}

\RN{This is why I said the results are muddy. Basically, there are two patterns. For prograde spin, $\Phi$ decreases with increasing $a_*$, and so does $\sqrt{\dot{M}}$, so the ratio, which gives $\phi_{\rm BH}$, remains roughly constant. On the other hand, for retrograde spin, $\Phi$ decreases a lot as you go from $a_*=0$ to $a_*=-0.9$, whereas $\sqrt{\dot{M}}$ is more or less constant. Hence we have a large decline in $\phi$. I am not sure there is any simple explanation in terms of flux transport. I suggest leaving out Figures \ref{fig:phi_r} and \ref{fig:Phi_Mdot} and the related discussion unless one of you has a strong reason for keeping it.}
